Snapping Matters: Context-Aware Onset Refinement for Automatic Music Transcription

Precise note-level annotations are critical for training automatic music transcription (AMT) systems, in particular note-onset labels, which form a core component of many recent AMT systems. However, high-quality annotations for real-world recordings are scarce. Sequence-level score--audio alignment methods such as dynamic time warping provide only coarse correspondence, making a local refinement step necessary. This refinement step, known as snapping, adjusts aligned score onsets using peaks in a neural onset posteriorgram and often determines whether weakly aligned score--audio pairs become usable training data at all. Despite its practical importance, snapping is typically treated as a simple post-processing heuristic and implemented with greedy local decisions. We present a systematic analysis of snapping strategies for training instrument-agnostic transcribers, demonstrating that snapping is essential for learning from weakly aligned data. Building on this, we formulate snapping as a per-pitch assignment problem and solve it via bipartite graph matching, yielding context-aware onset decisions under overlapping refinement windows and uncertain initial alignments. Extensive cross-dataset experiments across piano, chamber, and orchestral recordings show improved onset alignment and transcription accuracy over greedy snapping, with gains increasing for wider snapping windows and coarser initial alignments. Qualitative examples are provided on our project page: https://abhirupsaha8.github.io

==> commented.tex <==
% While onset or chroma features---whether derived from signal processing techniques~\cite{EwertMG09_HighResAudioSync_ICASSP,OezerKM21_SyncToolbox_ISMIR-LBD, MuellerOKPD21_SyncToolbox_JOSS} or neural features~\cite{ZeitlerMM24_Synchronization_ISMIR}---have demonstrated high robustness for alignment algorithms such as dynamic time warping (DTW), they are often insufficiently accurate for generating annotations suitable for transcription, in particular annotations regarding note onset timing, due to subtle expressive temporal variations in performance~\cite{MamanBermano22_UnalignedAMT_ICML, RileyED24_GuitarTranscription_ICASSP}.

% Training reliable transcribers for note detection depends heavily on the quality of temporal alignment between the score and audio. Since onsets are sparse and occur over short time intervals, frame-level precision (approximately 32\,ms in our case) is essential for effective learning. Even small misalignments can cause label uncertainty, leading to degraded transcription accuracy. Hence, achieving \textit{note-level alignment}, where each notated onset precisely corresponds to its acoustic realization, plays a critical role in AMT training.

% While synthetic datasets provide perfectly aligned ground truth, they fail to capture the expressive timing, dynamics, and acoustic complexity of real performances. Real-world recordings, on the other hand, exhibit variability that challenges alignment accuracy. To address this, several studies have proposed algorithms that align scores and performances either through signal-processing features, neural representations, or a combination of both.

% Signal-processing-based methods, such as those using chroma or DLNCO features~\cite{MuellerOKPD21_SyncToolbox_JOSS}, have long served as robust foundations for audio–score synchronization. For instance, ~\cite{HuD06_bootstrapOnset_ML} introduced an EM-based onset learning approach using weakly aligned data, while ~\cite{NiedermayerW10_AudioScoreAlign_ISMIR} proposed a multi-pass strategy that uses high-confidence anchor points for alignment refinement. ~\cite{ZeitlerMM24_Synchronization_ISMIR} demonstrated the strong cross-domain robustness of chroma features, particularly for coarse alignment tasks. 

% With the progress of neural models, several works have leveraged learned representations for improved alignment precision. ~\cite{KwonJN20_PianoTranscription_ISMIR} employed RNN-based features for piano transcription alignment, while ~\cite{MamanBermano22_UnalignedAMT_ICML} and ~\cite{YaffeMMB25_CountEM_ISMIR} extended this idea to multi-instrument music using neural onset features and histogram-based approaches, respectively. These methods demonstrate that neural features can yield fine-grained alignment adjustments where purely signal-based features may fall short.

% In this work, we propose a hybrid alignment framework that combines the strengths of both paradigms. We first perform \textit{coarse alignment} using signal-processing-based features following the approach of ~\cite{MuellerOKPD21_SyncToolbox_JOSS}, ensuring global temporal consistency. Subsequently, we apply \textit{local adjustment} using neural onset features to refine note-level precision. By systematically comparing these alignment strategies and their combinations, this paper provides a clearer understanding of how to best utilize existing methods for constructing high-quality, real-world training data for AMT.

% \textcolor{red}{TODO: Add figure for Coarse vs Note-level Alignment, add dataset overview and their limitations and particularly mention Ben's and Yaffe's method in more details.}
% This template can be downloaded from the \href{https://icmc2026.ligeti-zentrum.de/}{ICMC 2026 web site}\footnote{\href{https://icmc2026.ligeti-zentrum.de/}{https://icmc2026.ligeti-zentrum.de}}.

% In practice, when aligning a musical score to an audio recording of a performance of the same score, a good sequence-level alignment does not necessarily guarantee a good onset-level alignment. For example, if two note onsets occur within the same frame on the score timeline but occur in different frames in the audio timeline (as in arpeggios or similar expressive deviations), then any onset-level alignment induced directly from the sequence-level warping will necessarily assign an incorrect onset time to at least one of the notes.

% Still, if we denote the true latent note-level alignment by \(\mathcal{M}^*\), and denote the induced onset-level alignment by \(\mathcal{M}\), we can assume there exists some bound \(B\) on the error, such that
% \[
% |\mathcal{M}(n) - \mathcal{M}^*(n)| \le B, 
% \quad \forall\, n \in \mathcal{N}.
% \]

% Musical score timeline and physical timeline 
% \[
% \mathcal{T}_\mathrm{s} = \{1,\dots,T_\mathrm{s}\},\quad \mathcal{T}_\mathrm{a} = \{1,\dots,T_\mathrm{a}\}
% \]
% Sequence level alignment is a warping function \[\mathcal{W}: \mathcal{T}_\mathrm{s}\to \mathcal{T}_\mathrm{a}\] according to some frame-level similarity or some other method.

% Musical score represented as list of notes
% \[
% \mathcal{N} = \{n_k\}_{k=1}^N, \qquad 
% n_k = (p_k,\, t_k^{\mathrm{on}},\, t_k^{\mathrm{off}},\, i_k),
% \]

% a note-level alignment is a function
% \[
% \mathcal{M}^\mathrm{on} \times \mathcal{M}^\mathrm{off}: \mathcal{N}\to \mathcal{T}_\mathrm{a} \times \mathcal{T}_\mathrm{a}
% \]
% that maps each note to its onset time and offset time in the physical timeline.

% In this work, we focus on onset detection, therefore we consider an onset-level alignment to be a function:
% \[
% \mathcal{M}: \mathcal{N}\to \mathcal{T}_\mathrm{a}
% \]
% that maps each note to its onset time in the physical timeline.

% \[
% \{n_k\}_{k=1}^N, \qquad 
% n_k = (p_k,\, t_k^{\mathrm{on}},\, t_k^{\mathrm{off}},\, i_k),
% \]
% where each event is specified by its pitch \(p_k\), onset time \(t_k^{\mathrm{on}}\), offset time \(t_k^{\mathrm{off}}\), and instrument label \(i_k\). For simplicity, we assume $t_k^{\mathrm{on}},\, t_k^{\mathrm{off}}$ are already in physical time.
% From this representation

% \[
% M^{\mathrm{ac}}_{t,p} =
% \begin{cases}
% 1, & \exists\,k:\; p_k = p \\ 
%    & \quad \text{and } [tS,(t+1)S] \cap [t_k^{\mathrm{on}},t_k^{\mathrm{off}}] \neq \emptyset, \\[2pt]
% 0, & \text{otherwise}.
% \end{cases}
% \]

% \[
% M^{\mathrm{ac}}_{t,p}
% =\mathbf{1}\!\biggl\{
% \exists\,k:\;
% p_k = p
% \ \wedge\
% \bigl[tS,(t+1)S\bigr]\cap
% \bigl[t_k^{\mathrm{on}},t_k^{\mathrm{off}}\bigr]\neq\emptyset
% \biggr\}.
% \]

% \[
% M^{\mathrm{ac}}_{t,p} =
% \begin{cases}
% 1 &  \exists\, k \text{ s.t. } p_k = p 
% \text{ and } \\ 
% & (tS \in [t_k^{\mathrm{on}},\, t_k^{\mathrm{off}}]\text{ or } (t + 1)S \in [t_k^{\mathrm{on}},\, t_k^{\mathrm{off}}]), \\[4pt]
% 0 & \text{otherwise}.
% \end{cases}
% \]



% \[
% M^{\mathrm{on}}_{t,p} =
% \begin{cases}
% 1 & \exists\, k \text{ s.t. } p_k = p 
% \text{ and } t_k^{\mathrm{on}} \in [tS,\, tS + 1), \\[4pt]
% 0 & \text{otherwise}.
% \end{cases}
% \]

% Instrument-agnostic transcription aims to infer note activity without distinguishing between instruments. Although this task has been explored in prior work, it is often not stated in a fully explicit or formal manner. In this section, we provide such a definition, discuss challenges that arise from it, and detail simplifying assumptions used in this work.

% Starting from a representation of the musical score as a list of note events as in Equation~\ref{eq:note_list}, we derive a discretized piano roll  
% \(M \in [0,1]^{T_\mathrm{s} \times P}\), where \(T_\mathrm{s}\) and \(P\) denote the score's time and pitch resolution.

% We define the \emph{note onset piano roll}, which highlights only the note onsets (beginnings):
% \[
% M^{\mathrm{on}}_{t,p} =
% \begin{cases}
% 1, & \exists\,k:\; p_k = p \text{ and } t = t_k^\mathrm{on}, \\
% 0 & \text{otherwise}.
% \end{cases}
% \]

% Similarly, we can define the \emph{note activity piano roll}:
% \[
% M^{\mathrm{ac}}_{t,p} =
% \begin{cases}
% 1, & \exists\,k:\; p_k = p \text{ and } t_k^\mathrm{on} \le t \le  t_k^\mathrm{off}, \\
% 0, & \text{otherwise}.
% \end{cases}
% \]

% In this work, we focus on onset detection, therefore we denote $M = M^{\mathrm{on}}$.  


% \subsection{Obtaining Coarse Estimates}
% In order to perform snapping as described in the previous section, we require a coarse estimated matching \[\mathcal{M}_0: \mathcal{N}\to\mathcal{T}_\mathrm{a}.\]
% For this, we use a score--audio alignment algorithm, which provides a warping
% \[\mathcal{W}: \mathcal{T}_\mathrm{s}\to\mathcal{T}_\mathrm{a}\]
% of the score timeline $\mathcal{T}_\mathrm{s}$ into the audio timeline. For each pitch class $p$ with occurrences $\mathcal{N}$, this induces a coarse matching $\mathcal{M}_0:\mathcal{N}\to\mathcal{T}_\mathrm{a}$ defined by:
% \[
% \mathcal{M}_0(n) = \mathcal{W}(t(n))
% \]
% where $t(n)$ is the time in the score timeline in which the note $n$ occurs.

% The better the score--audio alignment, the smaller the error bound $B$ that is required. We experiment with different score--audio alignment algorithms, namely dynamic time warping (DTW) with signal-processing-based features, and a crude alignment algorithm---linear stretching of the score to the audio. We show our approach operates robustly using either of the latter (DTW and linear stretching), by adjusting the error bound $B$.




% We formulate the local-maximum adjustment (or \emph{snapping}) procedure as a \emph{graph-matching} problem, as illustrated in Figure~\ref{fig:overview}. 
% Let 
% \[
% \mathcal{M}_0: T_{\mathrm{s}} \to T_{\mathrm{a}}
% \]
% denote a coarse alignment between the \emph{score timeline} and the \emph{audio timeline}, which are both discrete:
% \[
% T_{\mathrm{s}} = \{1, \dots, M\},\quad T_{\mathrm{a}} = \{1, \dots, N\}.
% \]



% Assume a binary labeling function $Y: T_{\mathrm{s}} \to \{0,1\}$
% which identifies the subset of positively labeled score positions
% \[
% T_{\mathrm{s}}^{\mathrm{P}} = Y^{-1}(\{1\}).
% \]
% We further posit the existence of a latent, injective (one-to-one) ground-truth matching
% \[
% \mathcal{M}^* : T_{\mathrm{s}}^{\mathrm{P}} \to T_{\mathrm{a}}.
% \]

% We assume the coarse alignment $\mathcal{M}_0$ is locally accurate within a bounded temporal deviation $B$, i.e.,
% \[
% |\mathcal{M}_0(i) - \mathcal{M}^*(i)| \le B, 
% \quad \forall\, i \in T_{\mathrm{s}}^{\mathrm{P}}.
% \]

% For each score position \( i \in T_{\mathrm{s}}^{\mathrm{P}} \), 
% we define the set of admissible candidate matches as
% \[
% \Omega_i = 
% \bigl\{\, j \in T_{\mathrm{a}} \,\bigm|\, 
% |j - \mathcal{M}_0(i)| \le B \,\bigr\}.
% \]

% Given a learned posteriorgram
% \[
% f_\theta : T_{\mathrm{a}} \to [0,1],
% \]
% where \( f_\theta(j) \) represents the likelihood that \( j \) corresponds to a true match \( \mathcal{M}^*(i) \),
% we seek to refine the alignment within the admissible window.

% We define a weighted bipartite graph
% \[
% G = (V_{\mathrm{s}}, V_{\mathrm{a}}, E),
% \]
% with vertex sets $V_{\mathrm{s}} = T_{\mathrm{s}}^{\mathrm{P}}$ and $V_{\mathrm{a}} = \{1, \dots, N\}$, and edge set
% \[
% E = \{\, (i,j) \mid j \in \Omega_i \,\}.
% \]
% Each edge \((i,j)\) carries a weight $w_{i,j} = f_\theta(j)$, which quantifies the likelihood of aligning score position \( i \) to audio frame \( j \).
% For all \( j \notin \Omega_i \), we set \( w_{i,j} = 0 \).

% We seek the matching
% \[
% \widehat{\mathcal{M}} 
% = \arg\max_{\mathcal{M}}
% \sum_{i \in T_{\mathrm{s}}^{\mathrm{P}}} 
% w_{i, \mathcal{M}(i)}\]
% subject to the following constraints:
% \[
% \mathcal{M}(i) \in \Omega_i, 
% \quad \forall\, i \in T_{\mathrm{s}}^{\mathrm{P}},
% \]
% \[
% i_1 \ne i_2 
% \implies 
% \mathcal{M}(i_1) \ne \mathcal{M}(i_2),
% \quad \forall\, i_1, i_2 \in T_{\mathrm{s}}^{\mathrm{P}}.
% \]

% \input{tables/table}

% % Since candidate sets \(\Omega_i\) may overlap, a naïve local selection may yield a suboptimal global alignment. 
% % An optimal assignment can instead be obtained using classical algorithms for bipartite matching, such as those of Karp~\cite{karp1980algorithm} or Jonker and Volgenant~\cite{jonker1987shortest}.

% Since candidate sets \(\Omega_i\) may overlap, a naïve local selection may yield a suboptimal global alignment, as depicted in Figure~\ref{fig:overview}. 
% An optimal assignment can instead be obtained using classical algorithms for bipartite matching, such as those of ~\cite{karp1980algorithm, jonker1987shortest}.

% We denote the resulting snapping operator as
% \[
% \mathcal{BP}(f_\theta, Y, \mathcal{M}_0, B) = \widehat{\mathcal{M}}.
% \]





% We formulate local-maximum adjustment or "snapping" as a graph-matching problem. We assume some approximate or coarse alignment mapping $\mathcal{M}_0:T_{\mathrm{s}}\to T_{\mathrm{a}}$ between a score audio timeline $T_{\mathrm{s}}=\{1, \dots, M\}$ and an audio timeline $T_{\mathrm{a}}=\{1, \dots, N\}$. We assume there exists an assignment function or score label $Y:T_{\mathrm{s}}\to \{0, 1\}$, with a positive set $T_{\mathrm{s}}^{\mathrm{P}}=Y^{-1}(\{1\})$, and a latent true one-to-one (injective) assignment $\mathcal{M}^* :T_{\mathrm{s}}^{\mathrm{P}}\to T_a$. We assume the error can be bounded by some $B$, such that
% \[
% |\mathcal{M}_0(i) - \mathcal{M}^*(i)| \le B, \quad \forall i\in T_{\mathrm{s}}^{\mathrm{P}}.
% \]

% Therefore, we can define for each $i\in P$ the set of candidate corresponding matches:
% \[
% \Omega_i = \{\, j \in T_{\mathrm{a}} \mid |j - \mathcal{M}_0(i)| \le B \,\}.
% \]

% In addition, we have a posteriorgram
% \[
% f_\theta : T_{\mathrm{a}} \to [0, 1]
% \]
% where $f_\theta(j)$ predicts the likelihood that $\mathcal{M}^*(i)=j$ for some $i$. We define a bi-partite graph

% \[
% G = (V_{\mathrm{s}}, V_{\mathrm{a}}, E),
% \]
% where \(V_{\mathrm{s}} = T_{\mathrm{s}}^{\mathrm{P}}\) and \(V_{\mathrm{a}} = \{1, \dots, N\}\) are the score and audio vertex sets, and
% \[
% E = \{\, (i,j) \mid j \in \Omega_i \,\}
% \]
% is the set of admissible alignment edges.  
% Each edge \((i,j)\) carries a weight
% \[
% w_{i,j} = f_\theta(j)
% \]
% representing the likelihood of aligning score position \(i\) to audio frame \(j\). If $j\notin\Omega_i$ we set $w_{ij} = 0$. We then search for an alignment $\widehat{\mathcal{M}}$

% \[
% \widehat{\mathcal{M}} 
% = \arg\max_\mathcal{M} 
% \sum_{i=1}^{M} w_{i,\mathcal{M}(i)}
% \]
% subject to:
% \[
% \mathcal{M}: T_{\mathrm{s}}^{\mathrm{P}}\to T_{\mathrm{a}}, \quad 
% \mathcal{M}(i) \in \Omega_i, \quad \forall i \in T_{\mathrm{s}}^{\mathrm{P}}
% \]
% \[
% i_1 \neq i_2 \implies \mathcal{M}(i_1) \neq \mathcal{M}(i_2), \quad\forall i_1, i_2 \in T_{\mathrm{s}}^{\mathrm{P}}.
% \]
% If $\Omega_i$ intersect each other, a na\"{\i}ve solution may be suboptimal. An optimal solution can be obtained using algorithms proposed by~\cite{karp1980algorithm, jonker1987shortest}.

% We define
% \[
% \mathcal{BP}(f_\theta, Y) = \widehat{\mathcal{M}} 
% \]
% \textcolor{red}{TODO: Add figure for Bi-partite vs Greedy Match.}



% \subsection{Handling Evaluation Set Misalignment}
% Annotations for MAESTRO and SMD are highly accurate, with temporal precision on the order of 3\,ms, thanks to the use of the Disklavier. In contrast, evaluation sets for string and wind instruments exhibit lower timing accuracy. While the overall musical score labels generally match the audio recordings, note onset and offset times may contain temporal errors. In principle, snapping could also be applied to the evaluation set; however, since snapping is precisely what we aim to evaluate, doing so would introduce bias. Therefore, to account for small alignment errors, we use higher onset tolerance thresholds than the standard 50\,ms or compute metrics under an optimal global shift. The procedure for selecting these thresholds and shifts is described in the following paragraphs.

% \textbf{Tolerance Threshold Selection:} Thresholds were determined by examining the effect of increasing onset tolerance on F1 score. For each dataset, if a small increase in tolerance caused a sharp rise in F1, we selected the higher threshold, as lower performance under stricter thresholds may reflect annotation errors rather than transcriber inaccuracies. For instance, in ChoraleBricks, increasing the onset tolerance from 50\,ms to 100\,ms improves F1 by 15\%, and raising it further to 200\,ms yields an additional 3\% gain. We consider 200\,ms a reasonable estimate of human annotation error. For completeness, we also report transcription metrics at stricter 50\,ms and 100\,ms thresholds for all datasets in separate tables.

% \textbf{Tolerance Threshold Selection Procedure:} Thresholds were chosen by analyzing the effect of increasing onset tolerance on F1 score. For each dataset, if a small increase in tolerance resulted in a sharp rise in F1 score, we selected the higher threshold, as lower performance under stricter thresholds may reflect temporal errors in the annotations rather than transcriber inaccuracies. For example, in ChoraleBricks, increasing the onset tolerance from 50\,ms to 100\,ms improves the F1 score by 15\%, and increasing it further to 200\,ms provides an additional 3\% gain. We consider 200\,ms to be a reasonable estimate of human annotation error. For completeness, we also provide transcription metrics at the stricter 50\,ms and 100\,ms thresholds for all datasets in separate tables.

% \textbf{Global Shift Selection Procedure:} For URMP, we use the standard 50\,ms onset threshold. However, we observed that applying a global shift of up to 100\,ms to the reference annotations can improve the F1 score by up to 5\%. This likely arises from global misalignments between transcriber predictions and labels, due to human error or differing annotation policies. Accordingly, we report results for URMP both with the optimal global shift applied and without any shift.

% \subsection{Handling Evaluation Set Misalignment}
% Annotations for MAESTRO and SMD are highly accurate, with temporal precision on the order of 3\,ms, thanks to the use of the Disklavier. In contrast, evaluation sets for string and wind instruments do not have this level of timing accuracy. While the overall musical score labels are consistent with the audio recordings, note onset and offset times may contain temporal errors. To account for this, we adopt a more lenient tolerance for onset deviations than the standard 50\,ms. Specifically, we use 100\,ms threshold for PHENICX and 200\,ms for ChoraleBricks.

% \textbf{Threshold Selection Procedure:} We chose these threshold value in the following manner: For each dataset, if a small increase in onset tolerance resulted in a sharp rise in F1 score, we selected the higher threshold. This is because lower performance under a stricter threshold may reflect temporal errors in the annotations rather than inaccuracies of the transcriber. For instance, in ChoraleBricks, increasing the onset tolerance from 50\,ms to 100\,ms leads to a 15\% improvement in F1 score, and further increasing it to 200\,ms yields an additional 3\% gain. We consider 200\,ms to be a reasonable estimate of human annotation error. Nevertheless, for completeness, we also provide transcription metrics at the stricter 50\,ms and 100\,ms thresholds for all datasets in separate tables. 

% For the URMP dataset, we use the strict 50\,ms onset threshold. We observed, however, that applying a global shift of up to 100\,ms to the reference annotations can yield significant improvements of up to 5\% in F1 score. This improvement is likely due to global misalignments between the transcriber predictions and the labels, which may result from human error or different annotation policies. Accordingly, we report results for URMP both after applying the optimal global shift and without any global shift for completeness.

% (PHENICX, BSED, ChoraleBricks), or compute metrics under an optimal global shift of the reference (of up to 100\,ms) while keeping the stricter 50\,ms threshold (URMP).
%threshold under an optimal global shift of the reference within 100\,
% For URMP and PHENICX we use a 100\,ms threshold, for ChoraleBricks, a 200\,ms threshold, and for BSED a 1000\,ms threshold. The specific choice depends on the accuracy of each dataset's annotations. 
% % We describe the threshold
% % and global shift
% % selection process in detail, and
%  % \ben{In addition, we provide metrics under an optimal global shift of the reference (of up to 100\,ms) while keeping the stricter 50\,ms threshold. Finally, we also provide results for all datasets using the strict 50\,ms threshold.}
% % without applying any global shift, in Section~\ref{sec:threshold_selection}.

% % \subsection{Onset Threshold and Global Shift Selection}\label{sec:threshold_selection}
% % Thresholds were determined by examining the effect of increasing onset tolerance on F1 score.
% \textbf{Onset tolerance threshold selection} for each dataset among URMP, ChoraleBricks, and PHENICX was chosen as the smallest value in milliseconds from \(\{50, 100, 200\}\) at which the F1 score saturates: For each dataset, if a small increase in tolerance led to a sharp rise in F1, we selected the higher threshold, as lower performance under stricter thresholds may reflect temporal errors in the annotation rather than transcriber inaccuracies. For example, in ChoraleBricks, increasing the onset tolerance from 50\,ms to 100\,ms improves F1 by 15\%, and raising it further to 200\,ms yields an additional 3\% gain; we consider 200\,ms a reasonable estimate of human annotation error. In PHENICX, increasing the tolerance from 50\,ms to 100\,ms increases F1 by about 5\%, whereas further increasing it to 200\,ms yields less than a 1\% improvement; therefore, we retained the lower 100\,ms tolerance.
% In comparison to the string and wind datasets, for the piano datasets annotated using a Disklavier (MAESTRO, SMD), we observe that the F1 score already saturates at a 50\,ms threshold.

% For URMP, ChoraleBricks, and PHENICX, annotation was performed on separated monophonic tracks, enabling relatively high accuracy within 200\,ms.
% In contrast to URMP, ChoraleBricks, and PHENICX, where annotation was performed on separated monophonic tracks, enabling relatively high accuracy within 200\,ms, for BSED, score--audio alignment was performed on the full polyphonic track, which can yield larger timing errors; therefore, we use a tolerance of 1000\,ms. For completeness, we also report transcription metrics at the strict 50\,ms threshold for all datasets. In contrast, for the piano datasets annotated using a Disklavier (MAESTRO, SMD), we observe that the F1 score already saturates at 50\,ms.

% When compared to the piano datasets annotated using a Disklavier (MAESTRO, SMD), we observe that the F1 score already saturates at 50\,ms, even though the same alignment method was applied to the piano training data as to the other instruments. This may indicate that lower scores for the strict 50\,ms threshold than for the larger thresholds (e.g. 200\,ms) in URMP, ChoraleBricks, PHENICX, and BSED is due to annotation timing errors rather than actual lower performance.


% \textbf{Onset Tolerance Threshold Selection:}
% In general, the onset tolerance for each dataset was chosen as the smallest value at which the F1 score saturates: For each dataset, if a small increase in tolerance led to a sharp rise in F1, we selected the higher threshold, as lower performance under stricter thresholds may reflect temporal errors in the annotations rather than transcriber inaccuracies. For example, in ChoraleBricks, increasing the onset tolerance from 50\,ms to 100\,ms improves F1 by 15\%, and raising it further to 200\,ms yields an additional 3\% gain. We consider 200\,ms a reasonable estimate of human annotation error. In PHENICX, increasing the tolerance from 50\,ms to 100\,ms increases F1 by about 5\%, whereas further increasing it to 200\,ms yields less than a 1\% improvement; therefore, we retained the lower 100\,ms tolerance. While for URMP, ChoraleBricks, and PHENICX annotation was performed on separated monophonic tracks enabling relatively high accuracy within 200\,ms, for BSED score--audio alignment was performed on the full polyphonic track, which can yield larger timing errors, therefore we use a tolerance of 1000\,ms. Still, for completeness, we also report transcription metrics at the stricter 50\,ms and 100\,ms thresholds for all datasets.
% for URMP, ChoraleBricks, PHENICX and BSED.
% in Table~\ref{tab:choralebricks_tolerances}.

% Thresholds were determined by examining the effect of increasing onset tolerance on F1 score. For each dataset, if a small increase in tolerance led to a sharp rise in F1, we selected the higher threshold, as lower performance under stricter thresholds may reflect temporal errors in the annotations rather than transcriber inaccuracies. For example, in ChoraleBricks, increasing the onset tolerance from 50\,ms to 100\,ms improves F1 by 15\%, and raising it further to 200\,ms yields an additional 3\% gain. We consider 200\,ms a reasonable estimate of human annotation error. In PHENICX, increasing the tolerance from 50\,ms to 100\,ms increases F1 by about 5\%, whereas further increasing it to 200\,ms yields less than a 1\% improvement; therefore, we kept the lower 100\,ms tolerance. For completeness, we also report transcription metrics at the stricter 50\,ms and 100\,ms thresholds for both ChoraleBricks and PHENICX in Table~\ref{tab:choralebricks_tolerances}.

% \textbf{Global Shift Selection:} For URMP, we adopt the standard 50\,ms onset threshold under an optimal global shift of the reference, determined as follows. For each piece, we compute the F1 score between the predicted transcription and shifted versions of the reference transcription, ranging from $-100$\,ms to $100$\,ms in 10\,ms increments (20 shifts in total), and select the shift that maximizes the F1 score. This procedure can improve the F1 score by up to 5\%, likely due to global misalignments between transcriber predictions and annotations caused by human error or differing labeling conventions. This approach is stricter than simply increasing the onset tolerance threshold.

% We compare models trained with different alignment policies: We compare alignment based on bi-partite graph matching which we denote $\texttt{Bp}$, with the na\"ive greedy alignment which we denote $\texttt{Gr}$, commonly used in prior work. We apply snapping windows that range from 100\,ms to 60\,s (one minute). Two types of initial sequence-level alignments are considered: Dynamic Time Warping based on chroma and onset features~\cite{EwertMG09_HighResAudioSync_ICASSP,OezerKM21_SyncToolbox_ISMIR-LBD} denoted \texttt{DTW}, and linear stretching of the score to the audio timeline, denoted \texttt{LS}. Because LS can introduce substantial alignment errors, it requires large snapping windows to compensate. For example, \texttt{DTW-Bp} (0.64s) refers to graph-based snapping over 0.64 s windows applied after DTW alignment, whereas \texttt{Gr-LS} (60 s) denotes greedy snapping over 60 s windows applied after linear stretching.


% Lastly, another important effect that we see is that the larger the snapping window, the bigger the difference between greedy and graph-based snapping. This is evident  in cases where the initial sequence alignment is extremely coarse, using linear stretching of the the score to the audio. Such cases require large snapping windows to compensate. We see that in this case, even a 2-second window (\texttt{LS-Bp} 2s) is not sufficient for effective training. However, using extremely wide snapping windows of 20-60 s compensates for the gross alignment error: With such windows, when using graph-based snapping, we are still able to obtain considerable improvements over the synthetic baseline, despite the coarseness of the initial sequence-level alignment. For example, using 60-second windows, the F1 score improves on MAESTRO from 84.7 (\texttt{Synth}) to 88.3 (\texttt{LS-Bp} 60s). In addition, we see that the differences between graph-based and greedy-based snapping become larger in this case of extremely wide windows, with a consistent improvement of 2-5\% in recall and F1 score, when using the proposed graph-based approach. For example, on MAESTRO, applying greedy snapping after linear stretching (\texttt{LS-Gr} 60s) only mildly improves F1 score w.r.t. the synthetic baseline from 84.7 to 85.2, but decreases recall from 81.6 to 79.0. In contrast, applying graph-based snapping after linear stretching (\texttt{LS-Bp} 60s) improves recall and F1 w.r.t. greedy snapping (\texttt{LS-Gr} 60s), from 79.0 to 84.2 and from 85.2 to 88.3, respectively. These results show that graph-based snapping is much more robust than greedy snapping when using large snapping windows. This trend can also be seen, although more mildly, with the initial DTW alignment---on MAESTRO, the difference between greedy and graph is 0.3=89.9-89.6 for 0.096\,s, 0.9=90.1-89.2 for 0.64\,s, and 1.2=90.2-89.0 for 2\,s. This is not surprising at all, since larger windows naturally create more overlaps, making a greedy approach more prone to suboptimal solutions.

% This further confirms that larger windows cause more overlap between snapping windows and hence suboptimal solutions when following a greedy approach. Lastly, we see that snapping after DTW (\texttt{DTW-Bp 0.64s)} gives better results than after linear stretching (\texttt{LS-Bp 60s)}---0.90 vs. 0.88 on MAESTRO, and 0.86 vs. 0.81 on ChoraleBricks, indicating that a better initial sequence-level alignment enables using smaller snapping windows, thus providing better supervision.

% In this section we present piano transcription results for the models trained on MusicNet and evaluated on the MAESTRO test set, and on SMD. Results appear in Table~\ref{table:piano}.


==> custom_bib_old.tex <==
% Generated by IEEEtran.bst, version: 1.12 (2007/01/11)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{EwertMG09_HighResAudioSync_ICASSP}
S.~Ewert, M.~M{\"u}ller, and P.~Grosche, ``High Resolution Audio Synchronization Using Chroma Onset Features,'' in \emph{Proceedings of IEEE International Conference on Acoustics, Speech, and Signal Processing ({ICASSP})}, Taipei, Taiwan, 2009, pp. 1869--1872.

\bibitem{OezerKM21_SyncToolbox_ISMIR-LBD}
\BIBentryALTinterwordspacing
Y.~{\"O}zer, M.~Krause, and M.~M{\"u}ller, ``Using the Sync Toolbox for an Experiment on High-Resolution Music Alignment,'' in \emph{Demos and Late Breaking News of the International Society for Music Information Retrieval Conference ({ISMIR})}, Online, 2021. [Online]. Available: \url{https://archives.ismir.net/ismir2021/latebreaking/000025.pdf}
\BIBentrySTDinterwordspacing

\bibitem{MuellerOKPD21_SyncToolbox_JOSS}
M.~M{\"u}ller, Y.~{\"O}zer, M.~Krause, T.~Pr{\"a}tzlich, and J.~Driedger, ``{S}ync {T}oolbox: {A} {P}ython Package for Efficient, Robust, and Accurate Music Synchronization,'' \emph{Journal of Open Source Software ({JOSS})}, vol.~6, no.~64, pp. 3434:1--4, 2021.

\bibitem{ZeitlerMM24_Synchronization_ISMIR}
J.~Zeitler, B.~Maman, and M.~M{\"u}ller, ``Robust and Accurate Audio Synchronization Using Raw Features from Transcription Models,'' in \emph{Proceedings of the International Society for Music Information Retrieval Conference ({ISMIR})}, San Francisco, USA, 2024.

\bibitem{MamanBermano22_UnalignedAMT_ICML}
B.~Maman and A.~H. Bermano, ``Unaligned Supervision for Automatic Music Transcription in The Wild,'' in \emph{Proceedings of the International Conference on Machine Learning ({ICML})}, Baltimore, Maryland, USA, 2022, pp. 14\,918--14\,934.

\bibitem{RileyED24_GuitarTranscription_ICASSP}
X.~Riley, D.~Edwards, and S.~Dixon, ``High Resolution Guitar Transcription Via Domain Adaptation,'' in \emph{Proceedings of the {IEEE} International Conference on Acoustics, Speech, and Signal Processing ({ICASSP})}, Seoul, South Korea, 2024, pp. 1051--1055.

\bibitem{YaffeMMB25_CountEM_ISMIR}
J.~Yaffe, B.~Maman, M.~M{\"u}ller, and A.~Bermano, ``Count The Notes: Histogram-Based Supervision for Automatic Music Transcription,'' in \emph{Proceedings of the International Society for Music Information Retrieval Conference ({ISMIR})}, Daejeon, South Korea, 2025.

\bibitem{HuD06_bootstrapOnset_ML}
N.~Hu and R.~B. Dannenberg, ``Bootstrap learning for accurate onset detection,'' \emph{Machine Learning}, vol.~65, no. 2-3, pp. 457--471, 2006.

\bibitem{BenetosDGKK13_MusicTranscription_JIIS}
\BIBentryALTinterwordspacing
E.~Benetos, S.~Dixon, D.~Giannoulis, H.~Kirchhoff, and A.~Klapuri, ``Automatic music transcription: {C}hallenges and future directions,'' \emph{Journal of Intelligent Information Systems}, vol.~41, no.~3, pp. 407--434, 2013. [Online]. Available: \url{http://dx.doi.org/10.1007/s10844-013-0258-3}
\BIBentrySTDinterwordspacing

\bibitem{SmaragdisB03_MusicTranscriptionNMF_WASPAA}
P.~Smaragdis and J.~C. Brown, ``Non-Negative Matrix Factorization for Polyphonic Music Transcription,'' in \emph{Proceedings of the {IEEE} Workshop on Applications of Signal Processing to Audio and Acoustics ({WASPAA})}, 2003, pp. 177--180.

\bibitem{HawthorneESRSRE18_OnsetsFrames_ISMIR}
C.~Hawthorne, E.~Elsen, J.~Song, A.~Roberts, I.~Simon, C.~Raffel, J.~H. Engel, S.~Oore, and D.~Eck, ``Onsets and Frames: {D}ual-Objective Piano Transcription,'' in \emph{Proceedings of the International Society for Music Information Retrieval Conference, ({ISMIR})}, Paris, France, 2018, pp. 50--57.

\bibitem{HawthorneSRSHDE19_MAESTRO_ICLR}
\BIBentryALTinterwordspacing
C.~Hawthorne, A.~Stasyuk, A.~Roberts, I.~Simon, C.~A. Huang, S.~Dieleman, E.~Elsen, J.~H. Engel, and D.~Eck, ``Enabling Factorized Piano Music Modeling and Generation with the {MAESTRO} Dataset,'' in \emph{Proceedings of the International Conference on Learning Representations ({ICLR})}, New Orleans, Louisiana, USA, 2019. [Online]. Available: \url{https://openreview.net/forum?id=r1lYRjC9F7}
\BIBentrySTDinterwordspacing

\bibitem{KongEtAl21_HighResTranscription_TASLP}
\BIBentryALTinterwordspacing
Q.~Kong, B.~Li, X.~Song, Y.~Wan, and Y.~Wang, ``High-Resolution Piano Transcription With Pedals by Regressing Onset and Offset Times,'' \emph{{IEEE/ACM} Transactions of Audio, Speech, and Language Processing}, vol.~29, pp. 3707--3717, 2021. [Online]. Available: \url{https://doi.org/10.1109/TASLP.2021.3121991}
\BIBentrySTDinterwordspacing

\bibitem{ThickstunHK17_MusicNet_ICLR}
\BIBentryALTinterwordspacing
J.~Thickstun, Z.~Harchaoui, and S.~M. Kakade, ``Learning Features of Music from Scratch,'' in \emph{Proceedings of the International Conference on Learning Representations ({ICLR})}, Toulon, France, 2017. [Online]. Available: \url{https://openreview.net/forum?id=rkFBJv9gg}
\BIBentrySTDinterwordspacing

\bibitem{Mueller21_FMP_SPRINGER}
M.~M\"{u}ller, \emph{Fundamentals of Music Processing -- Using Python and Jupyter Notebooks}, 2nd~ed.\hskip 1em plus 0.5em minus 0.4em\relax Springer Verlag, 2021.

\bibitem{RileyGED2024_GAPS_ISMIR}
X.~Riley, Z.~Guo, and S.~Edwards, Drew abd~Dixon, ``GAPS: A Large and Diverse Classical Guitar Dataset and Benchmark Transcription Model,'' \emph{Proceedings of the International Society for Music Information Retrieval Conference (ISMIR), San Francisco, USA}, 2024.

\bibitem{StrahlM24_Semi_ISMIR}
S.~Strahl and M.~M{\"u}ller, ``Semi-Supervised Piano Transcription Using Pseudo-Labeling Techniques.'' in \emph{Proceedings of the International Society for Music Information Retrieval Conference ({ISMIR})}, 2024, pp. 173--181.

\bibitem{TamerOMS23_HighResViolinTranscription_ISMIR}
N.~C. Tamer, Y.~{\"O}zer, M.~M{\"u}ller, and X.~Serra, ``High-Resolution Violin Transcription using Weak Labels,'' in \emph{Proceedings of the International Society for Music Information Retrieval Conference ({ISMIR})}, Milan, Italy, 2023, pp. 223--230.

\bibitem{WuCS20_TranscriptionSelfattn_TASLP}
Y.~Wu, B.~Chen, and L.~Su, ``Multi-Instrument Automatic Music Transcription with Self-Attention-Based Instance Segmentation,'' \emph{{IEEE/ACM} Transactions on Audio, Speech and Language Processing}, vol.~28, pp. 2796--2809, 2020.

\bibitem{GardnerSMHE22_MultiTaskTranscription_ICLR}
J.~Gardner, I.~Simon, E.~Manilow, C.~Hawthorne, and J.~H. Engel, ``{MT3:} {M}ulti-Task Multitrack Music Transcription,'' in \emph{Proceedings of the International Conference on Learning Representations ({ICLR})}, Virtual, 2022.

\bibitem{WuWLLYGL24_Harmonic_ICME}
Y.~Wu, W.~Wei, D.~Li, M.~Li, Y.~Yu, Y.~Gao, and W.~Li, ``Harmonic Frequency-Separable Transformer for Instrument-Agnostic Music Transcription,'' in \emph{2024 IEEE International Conference on Multimedia and Expo (ICME)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2024, pp. 1--6.

\bibitem{karp1980algorithm}
R.~M. Karp, ``An algorithm to solve the m$\times$ n assignment problem in expected time O (mn log n),'' \emph{Networks}, vol.~10, no.~2, pp. 143--152, 1980.

\bibitem{jonker1987shortest}
R.~Jonker and A.~Volgenant, ``A shortest augmenting path algorithm for dense and sparse linear assignment problems,'' \emph{Computing}, vol.~38, no.~4, pp. 325--340, 1987.

\bibitem{MuellerKBA11_SMD_ISMIR-lateBreaking}
M.~M{\"u}ller, V.~Konz, W.~Bogler, and V.~Arifi-M{\"u}ller, ``Saarland Music Data ({SMD}),'' in \emph{Demos and Late Breaking News of the International Society for Music Information Retrieval Conference ({ISMIR})}, Miami, Florida, USA, 2011.

\bibitem{LiLDDS19_MultitrackDataset_TMM}
B.~Li, X.~Liu, K.~Dinesh, Z.~Duan, and G.~Sharma, ``Creating a Multitrack Classical Music Performance Dataset for Multimodal Music Analysis: Challenges, Insights, and Applications,'' \emph{{IEEE} Transactions on Multimedia}, vol.~21, no.~2, pp. 522--535, 2019.

\bibitem{BalkeBM25_ChoraleBricks_TISMIR}
S.~Balke, A.~Berndt, and M.~M{\"u}ller, ``{ChoraleBricks}: {A} Modular Multitrack Dataset for Wind Music Research,'' \emph{Transaction of the International Society for Music Information Retrieval ({TISMIR})}, vol.~8, no.~1, pp. 39--54, 2025.

\bibitem{LiemGS15_PHENICX_ICMWE}
C.~C.~S. Liem, E.~G{\'o}mez, and M.~Schedl, ``{PHENICX}: Innovating the Classical Music Experience,'' in \emph{Proceedings of the IEEE International Conference on Multimedia and Expo Workshops (ICMEW)}, Torino, Italy, June{\textendash}July 2015, pp. 1--4.

\bibitem{SchedlHTML16_PHENICX-SMM_CBMI}
M.~Schedl, D.~Hauger, M.~Tkalčič, M.~Melenhorst, and C.~C.~S. Liem, ``A Dataset of Multimedia Material about Classical Music: {PHENICX}-{SMM},'' in \emph{Proceedings of International Workshop on Content-Based Multimedia Indexing {(CBMI)}}, 2016, pp. 1--4.

\end{thebibliography}


==> tables/BSED_table.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccc|ccc}
\toprule
\multirow{2}{*}{Transcriber} & \multicolumn{3}{c}{BSED-DTW} & \multicolumn{3}{c}{BSED} \\
\cmidrule{2-7}
 & P & R & F1 & P & R & F1 \\
\midrule
\texttt{Synth} & 83.2 & 39.5 & 51.3 & 77.0 & 36.7 & 47.8 \\
\texttt{DTW} & 89.3 & 15.4 & 24.3 & 86.7 & 15.0 & 23.7 \\
\midrule
& \multicolumn{3}{c}{Previous Work} \\
\midrule
\texttt{DTW-Gr} (2s) & 81.6 & 59.9 & 67.2 & 76.7 & 56.6 & 63.4 \\
\texttt{DTW-Gr} (0.640s) & 78.9 & 62.4 & 67.6 & 73.4 & 58.6 & 63.4 \\
\texttt{DTW-Gr} (0.096s) & 83.9 & 53.4 & 62.3 & 79.6 & 50.7 & 59.3 \\
\texttt{LS-Gr} (60s) & 72.3 & 59.1 & 62.4 & 68.6 & 56.0 & 59.2 \\
\texttt{Hist} & 74.8 & 58.4 & 64.1 & 69.1 & 54.4 & 59.5 \\
\midrule
& \multicolumn{3}{c}{Ours} \\
\midrule
\texttt{DTW-Bp} (2s) & 79.7 & 62.2 & 67.8 & 74.6 & 58.5 & 63.7 \\
\texttt{DTW-Bp} (0.64s) & 81.4 & 63.8 & 69.6 & 75.6 & 59.6 & 64.9 \\
\texttt{DTW-Bp} (0.096s) & 84.4 & 53.9 & 63.4 & 79.0 & 51.0 & 59.8 \\
\texttt{LS-Bp} (60s) & 72.6 & 62.2 & 64.7 & 68.8 & 59.1 & 61.5 \\
\texttt{LS-Bp} (20s) & 73.3 & 62.0 & 64.9 & 69.0 & 58.8 & 61.4 \\
\texttt{LS-Bp} (10s) & 73.3 & 61.3 & 64.5 & 69.6 & 58.6 & 61.6 \\
\texttt{LS-Bp} (2s) & 74.1 & 47.4 & 55.0 & 68.9 & 44.5 & 51.6 \\

\bottomrule
\end{tabular}
\caption{Results for BSED-DTW with 500ms onset tolerance and BSED-Note with 100ms tolerance.}\label{table:orchestra}
\end{table}






==> tables/BSEDtable.tex <==
\begin{table}[!h]
\centering
\scalebox{0.9}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{50ms} & \multicolumn{3}{c}{1000ms} \\
\cmidrule{2-7}
& P & R & F1 & P & R & F1 \\
\midrule
\texttt{DTW} & 0.74 & 0.14 & 0.21 & 0.90 & 0.15 & 0.24 \\

% \texttt{BiP-DTW} (0.032s) & 0.70 & 0.20 & 0.28 & 0.78 & 0.21 & 0.31 \\

\texttt{BiP-DTW} (0.01s) & 0.73 & 0.47 & 0.55 & 0.86 & 0.55 & 0.64 \\

\texttt{BiP-DTW} (0.64s) & 0.68 & 0.54 & 0.59 & 0.82 & 0.65 & 0.71 \\

\texttt{BiP-DTW} (2s) & 0.67 & 0.53 & 0.58 & 0.81 & 0.63 & 0.69 \\

% \texttt{Gr-DTW} (0.032s) & 0.81 & 0.32 & 0.42 & 0.89 & 0.34 & 0.45 \\

\texttt{Gr-DTW} (0.01s) & 0.72 & 0.46 & 0.54 & 0.85 & 0.54 & 0.63 \\

\texttt{Gr-DTW} (0.64s) & 0.65 & 0.52 & 0.56 & 0.80 & 0.64 & 0.69 \\

\texttt{Gr-DTW} (2s) & 0.69 & 0.51 & 0.57 & 0.83 & 0.61 & 0.69 \\

\texttt{Hist} (30s) & 0.59 & 0.48 & 0.52 & 0.77 & 0.60 & 0.66 \\

\texttt{BiP-LS} (2s) & 0.62 & 0.40 & 0.46 & 0.77 & 0.49 & 0.57 \\

\texttt{BiP-LS} (10s) & 0.63 & 0.54 & 0.56 & 0.75 & 0.63 & 0.66 \\

\texttt{BiP-LS} (20s) & 0.62 & 0.53 & 0.55 & 0.75 & 0.64 & 0.67 \\

\texttt{BiP-LS} (60s) & 0.62 & 0.54 & 0.56 & 0.74 & 0.64 & 0.66 \\

\texttt{Gr-LS} (60s) & 0.61 & 0.50 & 0.53 & 0.74 & 0.61 & 0.64 \\

\texttt{Synth} & 0.58 & 0.29 & 0.37 & 0.85 & 0.40 & 0.52 \\
\bottomrule
\end{tabular}}
\caption{Note-level transcription results for different onset tolerances on BSED. We have used 50ms tolerance for their provided note-level-aligned labels and 1000ms tolerance for their provided sequence-aligned labels.}
\label{tab:bsed_tolerances}
\end{table}

==> tables/CBtable.tex <==
\begin{table}[!h]
\centering
\scalebox{0.73}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{50ms} & \multicolumn{3}{c|}{100ms} & \multicolumn{3}{c}{200ms} \\
\cmidrule{2-10}
& P & R & F1 & P & R & F1 & P & R & F1 \\
\midrule
\texttt{DTW} & 0.73 & 0.40 & 0.51 & 0.95 & 0.52 & 0.67 & 0.99 & 0.54 & 0.69 \\

% \texttt{BiP-DTW} (0.032 sec) & 0.77 & 0.36 & 0.47 & 0.89 & 0.42 & 0.55 & 0.91 & 0.42 & 0.56 \\

\texttt{BiP-DTW} (0.01s) & 0.78 & 0.64 & 0.70 & 0.93 & 0.76 & 0.83 & 0.96 & 0.78 & 0.85 \\

\texttt{BiP-DTW} (0.64s) & 0.76 & 0.66 & 0.70 & 0.91 & 0.80 & 0.85 & 0.94 & 0.83 & 0.88 \\

\texttt{BiP-DTW} (2s) & 0.75 & 0.67 & 0.70 & 0.90 & 0.80 & 0.84 & 0.93 & 0.83 & 0.87 \\

% \texttt{Gr-DTW} (0.032 sec) & 0.83 & 0.55 & 0.65 & 0.96 & 0.63 & 0.75 & 0.98 & 0.65 & 0.77 \\

\texttt{Gr-DTW} (0.01s) & 0.76 & 0.62 & 0.68 & 0.93 & 0.76 & 0.83 & 0.96 & 0.78 & 0.85 \\

\texttt{Gr-DTW} (0.64s) & 0.74 & 0.63 & 0.68 & 0.92 & 0.78 & 0.84 & 0.95 & 0.80 & 0.87 \\

\texttt{Gr-DTW} (2s) & 0.74 & 0.60 & 0.66 & 0.91 & 0.75 & 0.81 & 0.94 & 0.77 & 0.84 \\

\texttt{Hist} & 0.71 & 0.62 & 0.66 & 0.87 & 0.76 & 0.81 & 0.91 & 0.80 & 0.84 \\

\texttt{BiP-LS} (2s) & 0.78 & 0.54 & 0.63 & 0.90 & 0.62 & 0.73 & 0.93 & 0.64 & 0.75 \\

\texttt{BiP-LS} (10 sec) & 0.78 & 0.58 & 0.66 & 0.91 & 0.68 & 0.77 & 0.93 & 0.70 & 0.79 \\

\texttt{BiP-LS} (20 sec) & 0.71 & 0.60 & 0.64 & 0.86 & 0.73 & 0.78 & 0.90 & 0.76 & 0.82 \\

\texttt{BiP-LS} (60 sec) & 0.73 & 0.59 & 0.65 & 0.87 & 0.71 & 0.77 & 0.90 & 0.73 & 0.80 \\

\texttt{Gr-LS} (60 sec) & 0.66 & 0.63 & 0.64 & 0.79 & 0.76 & 0.77 & 0.82 & 0.79 & 0.80 \\

\texttt{Synth} & 0.73 & 0.60 & 0.66 & 0.86 & 0.71 & 0.77 & 0.88 & 0.73 & 0.80 \\
\bottomrule
\end{tabular}}
\caption{Note-level transcription results for different onset tolerances on ChoraleBricks.}
\label{tab:choralebricks_tolerances}
\end{table}


==> tables/PHENICXtable.tex <==
\begin{table}[!h]
\centering
\scalebox{0.73}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{50ms} & \multicolumn{3}{c|}{100ms} & \multicolumn{3}{c}{200ms} \\
\cmidrule{2-10}
& P & R & F1 & P & R & F1 & P & R & F1 \\
\midrule
\texttt{DTW} & 0.81 & 0.36 & 0.49 & 0.94 & 0.42 & 0.57 & 0.95 & 0.43 & 0.58 \\

% \texttt{BiP-DTW} (0.032 sec) & 0.82 & 0.41 & 0.55 & 0.86 & 0.43 & 0.58 & 0.87 & 0.44 & 0.58 \\

\texttt{BiP-DTW} (0.01s) & 0.83 & 0.57 & 0.68 & 0.88 & 0.61 & 0.72 & 0.89 & 0.62 & 0.73 \\

\texttt{BiP-DTW} (0.64s) & 0.79 & 0.58 & 0.67 & 0.85 & 0.63 & 0.72 & 0.86 & 0.63 & 0.73 \\

\texttt{BiP-DTW} (2s) & 0.81 & 0.58 & 0.67 & 0.87 & 0.62 & 0.72 & 0.88 & 0.62 & 0.73 \\

% \texttt{Gr-DTW} (0.032 sec) & 0.83 & 0.51 & 0.62 & 0.89 & 0.55 & 0.67 & 0.90 & 0.56 & 0.68 \\

\texttt{Gr-DTW} (0.01s) & 0.82 & 0.57 & 0.67 & 0.87 & 0.61 & 0.71 & 0.88 & 0.61 & 0.72 \\

\texttt{Gr-DTW} (0.64s) & 0.80 & 0.56 & 0.66 & 0.86 & 0.61 & 0.71 & 0.87 & 0.61 & 0.72 \\

\texttt{Gr-DTW} (2s) & 0.81 & 0.56 & 0.66 & 0.86 & 0.60 & 0.71 & 0.87 & 0.61 & 0.72 \\

\texttt{Hist} (30s) & 0.81 & 0.57 & 0.67 & 0.87 & 0.61 & 0.71 & 0.88 & 0.62 & 0.72 \\

\texttt{BiP-LS} (2s) & 0.82 & 0.35 & 0.48 & 0.86 & 0.37 & 0.51 & 0.87 & 0.37 & 0.52 \\

\texttt{BiP-LS} (10s) & 0.80 & 0.57 & 0.66 & 0.86 & 0.60 & 0.71 & 0.87 & 0.61 & 0.72 \\

\texttt{BiP-LS} (20 sec) & 0.80 & 0.57 & 0.66 & 0.85 & 0.61 & 0.71 & 0.86 & 0.62 & 0.72 \\

\texttt{BiP-LS} (60 sec) & 0.80 & 0.58 & 0.67 & 0.85 & 0.62 & 0.71 & 0.87 & 0.63 & 0.72 \\

\texttt{Gr-LS} (60 sec) & 0.74 & 0.58 & 0.65 & 0.79 & 0.62 & 0.69 & 0.81 & 0.64 & 0.71 \\

\texttt{Synth} & 0.79 & 0.51 & 0.62 & 0.84 & 0.55 & 0.66 & 0.85 & 0.56 & 0.67 \\
\bottomrule
\end{tabular}}
\caption{Note-level transcription results for different onset tolerances on PHENICX.}
\label{tab:phenicx_tolerances}
\end{table}

==> tables/URMPtable.tex <==
\begin{table}[!h]
\centering
\scalebox{0.95}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{w/ Global Shift} & \multicolumn{3}{c}{w/o Global Shift} \\
\cmidrule{2-7}
& P & R & F1 & P & R & F1 \\
\midrule
\texttt{DTW} & 0.91 & 0.59 & 0.71 & 0.91 & 0.58 & 0.70 \\
% \texttt{BiP-DTW} (0.032s) & 0.84 & 0.63 & 0.70 & 0.81 & 0.61 & 0.68 \\

\texttt{BiP-DTW} (0.01s) & 0.90 & 0.82 & 0.85 & 0.84 & 0.76 & 0.80 \\

\texttt{BiP-DTW} (0.64s) & 0.90 & 0.83 & 0.86 & 0.83 & 0.77 & 0.80 \\

\texttt{BiP-DTW} (2s) & 0.88 & 0.83 & 0.85 & 0.81 & 0.77 & 0.79 \\

% \texttt{Gr-DTW} (0.032s) & 0.93 & 0.74 & 0.81 & 0.90 & 0.72 & 0.80 \\
\texttt{Gr-DTW} (0.01s) & 0.91 & 0.80 & 0.85 & 0.85 & 0.75 & 0.79 \\

\texttt{Gr-DTW} (0.64s) & 0.90 & 0.82 & 0.86 & 0.82 & 0.75 & 0.78 \\

\texttt{Gr-DTW} (2s) & 0.88 & 0.81 & 0.84 & 0.80 & 0.74 & 0.77 \\

\texttt{Hist} & 0.85 & 0.82 & 0.84 & 0.81 & 0.77 & 0.79 \\

\texttt{BiP-LS} (2s) & 0.86 & 0.70 & 0.77 & 0.81 & 0.67 & 0.72 \\

\texttt{BiP-LS} (10s) & 0.87 & 0.78 & 0.82 & 0.82 & 0.73 & 0.77 \\

\texttt{BiP-LS} (20s) & 0.83 & 0.80 & 0.81 & 0.76 & 0.73 & 0.74 \\

\texttt{BiP-LS} (60s) & 0.84 & 0.78 & 0.81 & 0.78 & 0.72 & 0.75 \\

\texttt{Gr-LS} (60s) & 0.80 & 0.75 & 0.77 & 0.74 & 0.69 & 0.71 \\

\texttt{Synth} & 0.75 & 0.74 & 0.74 & 0.69 & 0.69 & 0.69 \\
\bottomrule
\end{tabular}}
\caption{Note-level transcription results for URMP with 50ms tolerance. One with an adjusted global shift and the other without during evaluation.}
\label{tab:urmp_shifts}
\end{table}

==> tables/main_table.tex <==
\begin{table*}[!h]
    \centering
    \setlength{\tabcolsep}{4pt}
    \scalebox{0.9}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
        \hline
        \multirow{2}{*}{Transcriber} 
        & \multicolumn{3}{c|}{MAESTRO \cite{HawthorneSRSHDE19_MAESTRO_ICLR}} 
        & \multicolumn{3}{c|}{PHENICX \cite{MironCBGJ16_OrchestraSourceSeparation_JECE}} 
        & \multicolumn{3}{c|}{BSED} 
        & \multicolumn{3}{c|}{ChoraleBricks \cite{BalkeBM25_ChoraleBricks_TISMIR}} 
        & \multicolumn{3}{c}{URMP \cite{LiLDDS19_MultitrackDataset_TMM}} \\
        \cline{2-16}
        & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\
        \hline \hline
        % $\mathcal{T}^{H}_{\text{MN}}$ 
        Histogram (30 sec) \cite{YaffeMMB25_CountEM_ISMIR}
        & 0.95 & 0.86 & \textbf{0.90} 
        & 0.87 & 0.61 & \textbf{0.71}
        & 0.59 & 0.48 & 0.52
        & 0.91 & 0.80 & 0.84
        & 0.85 & 0.82 & 0.84\\
        \hline
        % $\mathcal{T}^{G}_{\text{MN}}$ 
        Greedy Match (2 sec)
        & - & - & - 
        & - & - & -
        & - & - & -
        & - & - & -
        & - & - & - \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$ 
        Bi-partite (2 sec)
        & 0.94 & 0.87 & \textbf{0.90}
        & 0.84 & 0.61 & \textbf{0.71}
        & 0.67 & 0.53 & 0.58
        & 0.93 & 0.83 & \textbf{0.87}
        & 0.88 & 0.83 & \textbf{0.85} \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$ 
        Bi-partite (640 ms)
        & 0.95 & 0.86 & \textbf{0.90}
        & 0.85 & 0.63 & \textbf{0.72}
        & 0.68 & 0.54 & \textbf{0.59}
        & 0.94 & 0.83 & \textbf{0.88}
        & 0.90 & 0.83 & \textbf{0.86} \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$ 
        Bi-partite (96 ms)
        & \textbf{0.96} & 0.85 & \textbf{0.90}
        & \textbf{0.88} & 0.60 & \textbf{0.71}
        & \textbf{0.75} & 0.46 & 0.55
        & \textbf{0.96} & 0.78 & 0.85
        & 0.89 & 0.80 & \textbf{0.84} \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$ 
        Bi-partite (32 ms)
        & 0.96 & 0.75 & 0.84
        & 0.83 & 0.39 & 0.53
        & 0.72 & 0.17 & 0.25
        & 0.93 & 0.42 & 0.57
        & 0.90 & 0.63 & 0.73 \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$ 
        LM + Bi-partite (60 sec)
        & 0.93 & 0.84 & 0.88
        & 0.83 & 0.62 & 0.70
        & 0.69 & 0.51 & 0.56
        & 0.90 & 0.73 & 0.80
        & 0.85 & 0.74 & 0.79 \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$  
        LM + Bi-partite (20 sec)
        & 0.94 & 0.83 & 0.88
        & 0.83 & 0.59 & 0.69
        & 0.67 & 0.52 & 0.56
        & 0.90 & 0.76 & 0.82
        & 0.85 & 0.76 & 0.80 \\
        \hline
        % $\mathcal{T}^{B}_{\text{MN}}$  
        LM + Bi-partite (10 sec)
        & 0.94 & 0.80 & 0.87 
        & 0.85 & 0.58 & 0.68
        & 0.67 & 0.52 & 0.56
        & 0.93 & 0.70 & 0.79
        & 0.88 & 0.73 & 0.80 \\
        \hline
        % $\mathcal{T}^{S}_{\text{MN}}$ 
        DTW 
        & 0.96 & 0.50 & 0.63
        & 0.94 & 0.39 & 0.54
        & 0.58 & 0.09 & 0.14
        & 0.99 & 0.54 & 0.69
        & 0.92 & 0.58 & 0.69 \\
        \hline
        % $\mathcal{T}_{\text{Synth}}$ 
        Synth 
        & 0.88 & 0.82 & 0.85
        & 0.83 & 0.50 & 0.62
        & 0.69 & 0.27 & 0.37
        & 0.89 & 0.73 & 0.80
        & 0.73 & 0.70 & 0.71 \\
        \hline \hline
    \end{tabular}
    }
    \caption{Note-level transcription results across multiple datasets with a 50\,ms onset tolerance (100\,ms for PHENICX and 200\,ms for ChoraleBricks, accounting for alignment inaccuracies in the datasets). The transcribers are trained on MusicNet dataset~\cite{ThickstunHK17_MusicNet_ICLR}.}
    \label{tab:transcription}
\end{table*}

==> tables/orchestra_table_snapped_BSED.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccc|ccc}
\toprule
\multirow{2}{*}{Transcriber} & \multicolumn{3}{c}{BSED} & \multicolumn{3}{c}{PHENICX} \\
\cmidrule{2-7}
 & P & R & F1 & P & R & F1 \\
\midrule
\texttt{Synth} & 77.0 & 36.7 & 47.8 & 83.8 & 54.8 & 66.0 \\
\texttt{DTW} & 86.7 & 15.0 & 23.7 & 93.7 & 41.9 & 57.2 \\
\midrule
& \multicolumn{3}{c}{Previous Work} \\
\midrule
\texttt{DTW-Gr} (2s) & 76.7 & 56.6 & 63.4 & 85.8 & 60.0 & 70.4 \\
\texttt{DTW-Gr} (0.640s) & 73.4 & 58.6 & 63.4 & 85.5 & 60.3 & 70.4 \\
\texttt{DTW-Gr} (0.096s) & 79.6 & 50.7 & 59.3 & 87.1 & 60.6 & 71.2 \\
\texttt{LS-Gr} (60s) & 68.6 & 56.0 & 59.2 & 78.7 & 62.2 & 68.8 \\
\texttt{Hist} & 69.1 & 54.4 & 59.5 & 86.3 & 60.7 & 71.2 \\
\midrule
& \multicolumn{3}{c}{Ours} \\
\midrule
\texttt{DTW-Bp} (2s) & 74.6 & 58.5 & 63.7 & 86.3 & 61.5 & 71.5 \\
\texttt{DTW-Bp} (0.64s) & 75.6 & \textbf{59.6} & \textbf{64.9} & 84.4 & \textbf{62.3} & 71.5 \\
\texttt{DTW-Bp} (0.096s) & \textbf{79.0} & 51.0 & 59.8 & \textbf{87.6} & 60.9 & \textbf{71.7} \\
\texttt{LS-Bp} (60s) & 68.8 & 59.1 & 61.5 & 85.1 & 61.4 & 71.0 \\
\texttt{LS-Bp} (20s) & 69.0 & 58.8 & 61.4 & 84.9 & 60.7 & 70.5 \\
\texttt{LS-Bp} (10s) & 69.6 & 58.6 & 61.6 & 85.4 & 60.3 & 70.3 \\
\texttt{LS-Bp} (2s) & 68.9 & 44.5 & 51.6 & 85.6 & 36.4 & 50.8 \\
\bottomrule
\end{tabular}
\caption{Results for BSED and PHENICX.}\label{table:orchestra}
\end{table}





==> tables/perturbation_table_old.tex <==
% \begin{table}[t!]
%     \centering
%     \scalebox{0.8}{
%     \setlength{\tabcolsep}{4pt}
% \begin{tabular}{l|c|c|c|ccc}
%         \toprule
% \multicolumn{2}{c|}{} & Greedy & Bipartite & \multicolumn{3}{c}{No Snapping} \\
%         \cmidrule{5-7}
%         & \(w\) [s] & F1 & F1 & P & R & F1 \\
%         \midrule
%         \midrule
%         \multirow{4}{*}{\texttt{GT}}
%             & 0.032 & 100 & 100 & 100 & 100 & 100 \\
%             & 0.16 & 100 & 100 & 30.1 & 30.1 & 30.1 \\
%             & 0.48 & 100 & 100 & 16.7 & 16.7 & 16.7 \\
%             & 1.92 & 100 & 100 & 9.6 & 9.6 & 9.6 \\
%         \midrule
%         \multirowcell{4}{\texttt{BiP-DTW} \\ (0.64s)}
%             & 0.032 & 93.8 & 93.8 & &  &  \\
%             & 0.16 & 90.2 & 91.7 & & & \\
%             & 0.48 & 88.6 & 92.1 & & &  \\
%             & 1.92 & 85.8 & 91.1 & & & \\
%             \cmidrule{5-7}
%             \multicolumn{2}{c}{Transcr.} & & & 0.94 & 0.87 & 0.90 \\
%         \midrule
%         \multirow{4}{*}{\texttt{Synth}}
%             & 0.032 & 95.2 & 95.2 & & & \\
%             & 0.16 & 90.7 & 92.1 & & & \\
%             & 0.48 & 87.6 & 90.6 & & & \\
%             & 1.92 & 83.5 & 87.7 & & & \\
%             \cmidrule{5-7}
%             \multicolumn{2}{c}{Transcr} & & & 0.88 & 0.82 & 0.85 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Snapping evaluation on the MAESTRO test set across different perturbation windows \(w\).
%     Precision (P), Recall (R), and F1-scores are computed using onset tolerances of 50\,ms and 100\,ms. 
%     \uli{Is is maybe enough to report F1 scores here? Would shring the amount of large tables we have}
%     \uli{Also, we should use the same one-sided window definition as for the matching. Halve w(s) here}
%         % with a fixed peak-picking window of 1 frame. 
%     % $\mathcal{T}_{\text{Synth}}$ denotes the transcriber trained on synthetic data, 
%     % $\mathcal{T}_{\text{MN}}$ denotes the transcriber trained on the MusicNet dataset, and 
%     % $\mathcal{GT}_{\text{Features}}$ represents an ideal case where the transcriber is perfect and neural features are generated by smoothing the reference annotations.
%     }
%     \label{tab:perturbation}
% \end{table}


% Table 1: Greedy and Bipartite methods
\begin{table}[]
    \centering
\scalebox{0.78}{
\begin{tabular}{l|c|cc|ccc}
        \toprule
        & \multirow{2}{*}{\(w\) [s]} & \multicolumn{2}{c|}{Snapping} & \multicolumn{3}{c}{No Snapping} \\
        \cmidrule{3-4}\cmidrule{5-7}
        & & Greedy F1 & Bipartite F1 & P & R & F1 \\
        \midrule
        \multirow{4}{*}{\texttt{GT}}
            & 0.032 & 100 & 100 & 100 & 100 & 100 \\
            & 0.16 & 100 & 100 & 30.1 & 30.1 & 30.1 \\
            & 0.48 & 100 & 100 & 16.7 & 16.7 & 16.7 \\
            & 1.92 & 100 & 100 & 9.6 & 9.6 & 9.6 \\
        \midrule
        \multirowcell{4}{\texttt{BiP-DTW} \\ (0.64s)}
            & 0.032 & 93.8 & 93.8 & \multirow{4}{*}{95.0} & \multirow{4}{*}{95.9} & \multirow{4}{*}{90.1} \\
            & 0.16 & 90.2 & 91.7 & & & \\
            & 0.48 & 88.6 & 92.1 & & & \\
            & 1.92 & 85.8 & 91.1 & & & \\
        \midrule
        \multirow{4}{*}{\texttt{Synth}}
            & 0.032 & 95.2 & 95.2 & \multirow{4}{*}{88.4} & \multirow{4}{*}{81.6} & \multirow{4}{*}{84.7} \\
            & 0.16 & 90.7 & 92.1 & & & \\
            & 0.48 & 87.6 & 90.6 & & & \\
            & 1.92 & 83.5 & 87.7 & & & \\
        \bottomrule
\end{tabular}
}
    \caption{Evaluation of snapping on the perturbed MAESTRO test set across perturbation windows \(w\). Snapping methods show F1 only (since here P=R=F1 due to the known number of notes); no snapping shows P, R, and F1 for perturbed labels and transcriber outputs. Evaluation is always based on the true labels from MAESTRO.}
    \label{tab:placeholder}
\end{table}

==> tables/perturbation_table_old2.tex <==
\begin{table}[t!]
    \centering
    \scalebox{0.8}{
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|c|ccc|ccc}
        \toprule
\multicolumn{2}{c|}{} & \multicolumn{3}{c|}{Greedy} &
\multicolumn{3}{c}{Bipartite} \\
        \cmidrule{2-8}
        & \(w\) (s) & P & R & F1 & P & R & F1 \\
        \midrule

        \midrule
        \multirow{4}{*}{\texttt{GT}}
            & 0.032 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
            & 0.16 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
            & 0.48 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
            & 1.92 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
        \midrule
        \multirowcell{4}{\texttt{BiP-DTW} \\ (0.64s)}
        % \multirow{4}{*}{\texttt{BiP-DTW}}
            & 0.032 & 0.92 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
            & 0.16 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
            & 0.48 & 0.90 & 0.89 & 0.90 & 0.95 & 0.94 & 0.94 \\
            & 1.92 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.93 \\
            \cmidrule{2-8}
            & Transcr. & 0.94 & 0.87 & 0.90 & 0.95 & 0.87 & 0.91 \\
        \midrule
        \multirow{4}{*}{\texttt{Synth}}
            & 0.032 & 0.93 & 0.93 & 0.93 & 1.00 & 1.00 & 1.00 \\
            & 0.16 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
            & 0.48 & 0.89 & 0.88 & 0.88 & 0.94 & 0.93 & 0.93 \\
            & 1.92 & 0.87 & 0.86 & 0.86 & 0.92 & 0.90 & 0.91 \\
            \cmidrule{2-8}
            & Transcr & 0.88 & 0.82 & 0.85 & 0.89 & 0.82 & 0.85 \\
        \midrule
        \multirow{4}{*}{\texttt{No Snapping}}
            & 0.032 & 100 & 100 & 100 & 100 & 100 & 100 \\
            & 0.16  & 30.1 & 30.1 & 30.1 & 30.1 & 30.1 &  30.1 \\
            & 0.48  & 16.7 & 16.7 & 16.7 & 16.7 & 16.7 & 16.7 \\
            & 1.92  &  9.6 &9.6 & 9.6 &9.6 &9.6 & 9.6 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Snapping evaluation on the MAESTRO test set across different perturbation windows \(w\).
    Precision (P), Recall (R), and F1-scores are computed using onset tolerances of 50\,ms and 100\,ms. 
    \uli{Is is maybe enough to report F1 scores here? Would shring the amount of large tables we have}
    \uli{Also, we should use the same one-sided window definition as for the matching. Halve w(s) here}
        % with a fixed peak-picking window of 1 frame. 
    % $\mathcal{T}_{\text{Synth}}$ denotes the transcriber trained on synthetic data, 
    % $\mathcal{T}_{\text{MN}}$ denotes the transcriber trained on the MusicNet dataset, and 
    % $\mathcal{GT}_{\text{Features}}$ represents an ideal case where the transcriber is perfect and neural features are generated by smoothing the reference annotations.
    }
    \label{tab:perturbation}
\end{table}



% \begin{table*}[!h]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{l|c|c|ccc|ccc}
%         \hline
%         \textbf{Transcriber} &
%         \textbf{Perturbation Window (Frames)} &
%         \textbf{Peak-Picking Window (Frames)} &
%         \multicolumn{3}{c|}{\textbf{50\,ms}} &
%         \multicolumn{3}{c}{\textbf{100\,ms}} \\
%         \cline{4-9}
%         & & & P & R & F1 & P & R & F1 \\
%         \hline \hline
%         \multirow{16}{*}{$\mathcal{GT}_{\text{Features}}$}
%             & 0.064 & 0 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 1 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 2 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 3 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
%             \cline{2-9}
%             & 0.32 & 0 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.32 & 0.064 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.32 & 2 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.32 & 3 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             \cline{2-9}
%             & 0.96 & 0 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.96 & 0.064 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.96 & 2 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.96 & 3 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             \cline{2-9}
%             & 3.84 & 0 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 3.84 & 0.064 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 3.84 & 2 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 3.84 & 3 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             \cline{2-9}
%         \hline
%         \multirow{16}{*}{$\mathcal{T}_{\text{MN}}$}
%             & 0.064 & 0 & 0.92 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 1 & 0.92 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 2 & 0.92 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 3 & 0.93 & 0.93 & 0.93 & 1.00 & 1.00 & 1.00 \\
%             \cline{2-9}
%             & 0.32 & 0 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.32 & 0.064 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.32 & 2 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.32 & 3 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.93 \\
%             \cline{2-9}
%             & 0.96 & 0 & 0.90 & 0.89 & 0.90 & 0.95 & 0.94 & 0.94 \\
%             & 0.96 & 0.064 & 0.90 & 0.89 & 0.90 & 0.95 & 0.94 & 0.94 \\
%             & 0.96 & 2 & 0.90 & 0.89 & 0.90 & 0.95 & 0.94 & 0.94 \\
%             & 0.96 & 3 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.94 \\
%             \cline{2-9}
%             & 3.84 & 0 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.93 \\
%             & 3.84 & 0.064 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.93 \\
%             & 3.84 & 2 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.93 \\
%             & 3.84 & 3 & 0.89 & 0.88 & 0.88 & 0.93 & 0.92 & 0.93 \\
%             \cline{2-9}
%         \hline
%         \multirow{16}{*}{$\mathcal{T}_{\text{Synth}}$}
%             & 0.064 & 0 & 0.93 & 0.93 & 0.93 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 1 & 0.93 & 0.93 & 0.93 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 2 & 0.92 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
%             & 0.064 & 3 & 0.93 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
%             \cline{2-9}
%             & 0.32 & 0 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.32 & 0.064 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.32 & 2 & 0.89 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.32 & 3 & 0.89 & 0.88 & 0.88 & 0.94 & 0.93 & 0.93 \\
%             \cline{2-9}
%             & 0.96 & 0 & 0.89 & 0.88 & 0.88 & 0.94 & 0.93 & 0.93 \\
%             & 0.96 & 0.064 & 0.89 & 0.88 & 0.88 & 0.94 & 0.93 & 0.93 \\
%             & 0.96 & 2 & 0.89 & 0.88 & 0.88 & 0.94 & 0.93 & 0.93 \\
%             & 0.96 & 3 & 0.88 & 0.87 & 0.88 & 0.93 & 0.92 & 0.93 \\
%             \cline{2-9}
%             & 3.84 & 0 & 0.87 & 0.86 & 0.86 & 0.92 & 0.90 & 0.91 \\
%             & 3.84 & 0.064 & 0.87 & 0.86 & 0.86 & 0.92 & 0.90 & 0.91 \\
%             & 3.84 & 2 & 0.87 & 0.86 & 0.87 & 0.92 & 0.91 & 0.91 \\
%             & 3.84 & 3 & 0.87 & 0.86 & 0.86 & 0.91 & 0.90 & 0.91 \\
%             \cline{2-9}
%         \hline
%     \end{tabular}
%     }
%     \caption{Comparison of MAESTRO-Test set alignment results for different transcribers across all combinations of perturbation and peak-picking windows. Precision (P), Recall (R), and F1-scores are computed using onset tolerances of 50\,ms and 100\,ms.}
%     \label{tab:tau_results}
% \end{table*}



% \begin{table*}[!h]
%     \centering
%     \scalebox{0.9}{
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|c|ccc|ccc}
%         \hline
%         \textbf{Transcriber} &
%         \textbf{Perturbation Window (Frames)} &
%         \multicolumn{3}{c|}{\textbf{Alignment Results (50\,ms)}} &
% \multicolumn{3}{c}{\textbf{Alignment Results (100\,ms)}} \\
%         \cline{3-8}
%         & & P & R & F1 & P & R & F1 \\
%         \hline \hline
%         \multirow{4}{*}{$\mathcal{GT}_{\text{Features}}$}
%             & 0.064 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
%             & 0.32 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 0.96 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%             & 3.84 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 \\
%         \hline
%         \multirow{4}{*}{$\mathcal{T}_{\text{MN}}$}
%             & 0.064 & 0.92 & 0.92 & 0.92 & 1.00 & 1.00 & 1.00 \\
%             & 0.32 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.96 & 0.90 & 0.89 & 0.90 & 0.95 & 0.94 & 0.94 \\
%             & 3.84 & 0.89 & 0.88 & 0.89 & 0.94 & 0.93 & 0.93 \\
%         \hline
%         \multirow{4}{*}{$\mathcal{T}_{\text{Synth}}$}
%             & 0.064 & 0.93 & 0.93 & 0.93 & 1.00 & 1.00 & 1.00 \\
%             & 0.32 & 0.90 & 0.89 & 0.89 & 0.95 & 0.94 & 0.94 \\
%             & 0.96 & 0.89 & 0.88 & 0.88 & 0.94 & 0.93 & 0.93 \\
%             & 3.84 & 0.87 & 0.86 & 0.86 & 0.92 & 0.90 & 0.91 \\
%         \hline
%     \end{tabular}
%     }
%     \caption{Comparison of MAESTRO-Test set alignment results for different transcribers across perturbation windows with a fixed peak-picking window of 1 frame. 
%     Precision (P), Recall (R), and F1-scores are computed using onset tolerances of 50\,ms and 100\,ms. 
%     $\mathcal{T}_{\text{Synth}}$ denotes the transcriber trained on synthetic data, 
%     $\mathcal{T}_{\text{MN}}$ denotes the transcriber trained on the MusicNet dataset, and 
%     $\mathcal{GT}_{\text{Features}}$ represents an ideal case where the transcriber is perfect and neural features are generated by smoothing the reference annotations.}
%     \label{tab:perturbation}
% \end{table*}



==> tables/perturbation_table_t.tex <==

\begin{table}[]
    \centering
\scalebox{0.78}{
\begin{tabular}{l|c|cc|ccc}
        \toprule
        & \multirow{2}{*}{\(w\) [s]} & \multicolumn{2}{c|}{Snapping} & \multicolumn{3}{c}{No Snapping} \\
        \cmidrule{3-4}\cmidrule{5-7}
        & & Greedy & Bipartite & P & R & F1 \\
        \midrule
        \multirow{4}{*}{\texttt{GT}}
            & 0.032 & 100 & 100 & 100 & 100 & 100 \\
            & 0.16 & 100 & 100 & 30.1 & 30.1 & 30.1 \\
            & 0.48 & 100 & 100 & 16.7 & 16.7 & 16.7 \\
            & 1.92 & 100 & 100 & 9.6 & 9.6 & 9.6 \\
        \midrule
        \multirowcell{4}{\texttt{BiP-DTW} \\ (0.64s)}
            & 0.032 & 93.8 & 93.8 & \multirow{4}{*}{95.0} & \multirow{4}{*}{95.9} & \multirow{4}{*}{90.1} \\
            & 0.16 & 90.2 & 91.7 & & & \\
            & 0.48 & 88.6 & 92.1 & & & \\
            & 1.92 & 85.8 & 91.1 & & & \\
        \midrule
        \multirow{4}{*}{\texttt{Synth}}
            & 0.032 & 95.2 & 95.2 & \multirow{4}{*}{88.4} & \multirow{4}{*}{81.6} & \multirow{4}{*}{84.7} \\
            & 0.16 & 90.7 & 92.1 & & & \\
            & 0.48 & 87.6 & 90.6 & & & \\
            & 1.92 & 83.5 & 87.7 & & & \\
        \bottomrule
\end{tabular}
}
    \caption{Evaluation of snapping on the perturbed MAESTRO test set across perturbation windows \(w\). Snapping methods show F1 only (since here P=R=F1 due to the known number of notes); no snapping shows P, R, and F1 for perturbed labels and transcriber outputs. Evaluation is always based on the true labels from MAESTRO.}
    \label{table:perturbation}
\end{table}

==> tables/table.tex <==
\begin{table*}[t!]
    \centering
    \scalebox{0.88}{
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lccc|ccc|ccc|ccc|ccc|ccc}
    % \begin{tabular}{lcccccccccccccccccc}
        \toprule
        \multirow{2}{*}{Transcriber} & \multicolumn{3}{c}{MAESTRO \cite{HawthorneSRSHDE19_MAESTRO_ICLR}} & \multicolumn{3}{c}{PHENICX \cite{MironCBGJ16_OrchestraSourceSeparation_JECE}} & \multicolumn{3}{c}{BSED} & \multicolumn{3}{c}{ChoraleBricks \cite{BalkeBM25_ChoraleBricks_TISMIR}} & \multicolumn{3}{c}{URMP \cite{LiLDDS19_MultitrackDataset_TMM}} & \multicolumn{3}{c}{SMD \cite{MuellerKBA11_SMD_ISMIR-lateBreaking}}
        \\ \cmidrule{2-19}
        & P & R & F1         & P & R & F1         & P & R & F1         & P & R & F1         & P & R & F1         & P & R & F1 \\
        \midrule
        \texttt{Synth} & 0.88 & 0.82 & 0.85 & 0.84 & 0.55 & 0.66 & 0.58 & 0.29 & 0.37 & 0.88 & 0.73 & 0.80 & 0.75 & 0.74 & 0.74 & 0.93 & 0.86 & 0.89 \\
        \texttt{DTW} & 0.97 & 0.49 & 0.62 & 0.94 & 0.42 & 0.57 & 0.74 & 0.14 & 0.21 & 0.99 & 0.54 & 0.69 & 0.91 & 0.59 & 0.71 & 0.96 & 0.56 & 0.69 \\


\midrule
        & \multicolumn{18}{c}{Previous Work} \\
        \midrule
        
        \cite{MamanBermano22_UnalignedAMT_ICML} \texttt{Gr-DTW} (2s) & 0.94 & 0.85 & 0.89 & 0.86 & 0.60 & 0.71 & 0.69 & 0.51 & 0.57 & 0.94 & 0.77 & 0.85 & 0.88 & 0.81 & 0.84 & 0.97 & 0.88 & 0.92 \\
        \cite{MamanBermano22_UnalignedAMT_ICML} \texttt{Gr-DTW} (0.64s) & 0.94 & 0.85 & 0.89 & 0.86 & 0.61 & 0.71 & 0.65 & 0.52 & 0.56 & 0.95 & 0.80 & 0.87 & 0.90 & 0.82 & \textbf{0.86} & 0.98 & 0.87 & 0.92 \\
        \cite{MamanBermano22_UnalignedAMT_ICML} \texttt{Gr-DTW} (0.1s) & 0.96 & 0.85 & \textbf{0.90} & 0.87 & 0.61 & 0.71 & 0.72 & 0.46 & 0.54 & 0.96 & 0.78 & 0.85 & 0.91 & 0.80 & 0.85 & 0.98 & 0.86 & 0.91 \\
        % \texttt{Gr-DTW} (0.032s) & 0.97 & 0.77 & 0.85 & 0.89 & 0.55 & 0.67 & 0.81 & 0.32 & 0.42 & 0.98 & 0.65 & 0.77 & 0.93 & 0.74 & 0.81 & 0.96 & 0.80 & 0.87 \\
        
        \cite{MamanBermano22_UnalignedAMT_ICML} \texttt{Gr-LS} (60s) & 0.93 & 0.79 & 0.85 & 0.79 & 0.62 & 0.69 & 0.61 & 0.50 & 0.53 & 0.82 & 0.79 & 0.80 & 0.80 & 0.75 & 0.77 & 0.95 & 0.85 & 0.89 \\
        \cite{YaffeMMB25_CountEM_ISMIR} \texttt{Hist} & 0.95 & 0.86 & \textbf{0.90} & 0.87 & 0.61 & 0.71 & 0.59 & 0.48 & 0.52 & 0.91 & 0.80 & 0.84 & 0.85 & 0.82 & 0.84 & 0.98 & 0.88 & \textbf{0.93} \\
        
        \midrule
        & \multicolumn{18}{c}{Ours} \\
        \midrule
        \texttt{BiP-DTW} (2s) & 0.94 & 0.87 & \textbf{0.90} & 0.87 & 0.62 & \textbf{0.72} & 0.67 & 0.53 & 0.58 & 0.93 & 0.83 & 0.87 & 0.88 & 0.83 & 0.85 & 0.98 & 0.88 & \textbf{0.93} \\
        \texttt{BiP-DTW} (0.64s) & 0.95 & 0.86 & \textbf{0.90} & 0.85 & 0.63 & \textbf{0.72} & 0.68 & 0.54 & \textbf{0.59} & 0.94 & 0.83 & \textbf{0.88} & 0.90 & 0.83 & \textbf{0.86} & 0.98 & 0.88 & 0.92 \\
        \texttt{BiP-DTW} (0.1s) & 0.96 & 0.85 & \textbf{0.90} & 0.88 & 0.61 & \textbf{0.72} & 0.73 & 0.47 & 0.55 & 0.96 & 0.78 & 0.85 & 0.90 & 0.82 & 0.85 & 0.98 & 0.87 & 0.92 \\
        % \texttt{BiP-DTW} (0.032s) & 0.97 & 0.75 & 0.84 & 0.86 & 0.43 & 0.58 & 0.70 & 0.20 & 0.28 & 0.91 & 0.42 & 0.56 & 0.84 & 0.63 & 0.70 & 0.97 & 0.81 & 0.88 \\

\texttt{BiP-LS} (60s) & 0.93 & 0.84 & 0.88 & 0.85 & 0.62 & 0.71 & 0.62 & 0.54 & 0.56 & 0.90 & 0.73 & 0.80 & 0.84 & 0.78 & 0.81 & 0.97 & 0.88 & 0.92 \\
        \texttt{BiP-LS} (20s) & 0.94 & 0.83 & 0.88 & 0.85 & 0.61 & 0.71 & 0.62 & 0.53 & 0.55 & 0.90 & 0.76 & 0.82 & 0.83 & 0.80 & 0.81 & 0.98 & 0.87 & 0.92 \\
        \texttt{BiP-LS} (10s) & 0.94 & 0.80 & 0.87 & 0.86 & 0.60 & 0.71 & 0.63 & 0.54 & 0.56 & 0.93 & 0.70 & 0.79 & 0.87 & 0.78 & 0.82 & 0.98 & 0.86 & 0.91 \\
        \texttt{BiP-LS} (2s) & 0.95 & 0.52 & 0.65 & 0.86 & 0.37 & 0.51 & 0.62 & 0.40 & 0.46 & 0.93 & 0.64 & 0.75 & 0.86 & 0.70 & 0.77 & 0.96 & 0.64 & 0.74 \\
        
        
        \bottomrule
    \end{tabular}
    }
    \caption{
    Note-level transcription results (onsets within a temporal threshold) in a cross-dataset evaluation. Models are trained on MusicNet (except for the \texttt{Synth} baseline) and evaluated on other datasets. Reported metrics are note-level precision (P), recall (R), and F1-score (F1).
    % Note-level (onset-only, no offset) transcription results across multiple datasets. 
    % Onset tolerances are 50\,ms for MAESTRO, 100\,ms for PHENICX, 50\,ms for BSED, 200\,ms for ChoraleBricks, and 50\,ms for URMP to account for dataset-specific alignment inaccuracies. All transcribers are trained on the MusicNet dataset~\cite{ThickstunHK17_MusicNet_ICLR} except for Synth, which is trained on synthetic data. 
    % The transcribers use a combination of coarse alignment and local adjustment techniques:
    % - \texttt{BiP-DTW} (Xs): DTW for coarse alignment, bipartite matching for local adjustment with a window of XSonds on both sides. 
    % - DTW + Histogram (Xs): DTW for coarse alignment, histogram-based local adjustment with window XSonds. 
    % - \texttt{BiP-LS} (Xs): Linear mapping (LM) for coarse alignment, bipartite matching for local adjustment with window XSonds.  
    % Bolded values indicate the highest F1-score per dataset.
    }

    \label{tab:transcription}
\end{table*}

